Sorting Short Keys in Circuits of Size o(n log n)

We consider the classical problem of sorting an input array containing $n$ elements, where each element is described with a $k$-bit comparison-key and a $w$-bit payload. A long-standing open problem is whether there exist $(k + w) \cdot o(n \log n)$-sized boolean circuits for sorting. We show that one can overcome the $n\log n$ barrier when the keys to be sorted are short. Specifically, we prove that there is a circuit with $(k + w) \cdot O(n k) \cdot \poly(\log^*n - \log^* (w + k))$ boolean gates capable of sorting any input array containing $n$ elements, each described with a $k$-bit key and a $w$-bit payload. Therefore, if the keys to be sorted are short, say, $k < o(\log n)$, our result is asymptotically better than the classical AKS sorting network (ignoring $\poly\log^*$ terms); and we also overcome the $n \log n$ barrier in such cases. Such a result might be surprising initially because it is long known that comparator-based techniques must incur $\Omega(n \log n)$ comparator gates even when the keys to be sorted are only $1$-bit long (e.g., see Knuth's "Art of Programming" textbook). To the best of our knowledge, we are the first to achieve non-trivial results for sorting circuits using non-comparison-based techniques. We also show that if the Li-Li network coding conjecture is true, our upper bound is optimal, barring $\poly\log^*$ terms, for every $k$ as long as $k = O(\log n)$.

==> Makefile <==
# Switched this back to bibtex because the current version of crosstex
# seems to have a bug causing incorrect capitalization in the titles.

LATEX=pdflatex
TEXFLAGS=

TARGET=compaction-circuit.pdf 
TARGET2=main-smallkey-sort.pdf 

all: $(TARGET) $(TARGET2)

$(TARGET): $(TARGET:.pdf=.tex) *.tex *.bib Makefile
	$(LATEX) $(TEXFLAGS) $<
#	$(LATEX) $(TEXFLAGS) $<
	bibtex $(basename $<)
#	bibtex $(basename $<)
	$(LATEX) $(TEXFLAGS) $<
#	$(LATEX) $(TEXFLAGS) $<

$(TARGET2): $(TARGET2:.pdf=.tex) *.tex *.bib Makefile
	$(LATEX) $(TEXFLAGS) $<
	$(LATEX) $(TEXFLAGS) $<
	bibtex $(basename $<)
	bibtex $(basename $<)
	$(LATEX) $(TEXFLAGS) $<
	$(LATEX) $(TEXFLAGS) $<
	


full: $(TARGET:.pdf=.tex) *.tex *.bib Makefile
	$(LATEX) $(TEXFLAGS) $<
	$(LATEX) $(TEXFLAGS) $<
	bibtex $(basename $<)
	bibtex $(basename $<)
	$(LATEX) $(TEXFLAGS) $<
	$(LATEX) $(TEXFLAGS) $<
	

test: test-fonts test-info

test-fonts: $(TARGET)
	pdffonts $<

test-info: $(TARGET)
	pdfinfo $<

print: $(TARGET)
	pdftops $< - | lpr -P lws510

view: $(TARGET)
	kpdf $<

clean:
	rm -f $(TARGET) *.log *.aux *.bbl *.blg *.out *.bak .*.xtx.cache parsetab.py \#*\# *~


==> intro.tex <==
% !TEX root = compaction-circuit.tex
%\tableofcontents


\section{Introduction}
\label{sec:intro}

Compaction (also called tight compaction) 
is the following problem: given an input array consisting of $n$ elements
each of bit-width $w$ where a subset of the elements are marked as {\it distinguished},
output a permutation of the input array where 
all the distinguished elements are moved to the front, and all non-distinguished elements
moved to the end. 
Compaction can be viewed as a restricted form of sorting: essentially we would like
to sort an array of input elements each marked with a 1-bit key.
Compaction is a fundamental
algorithmic building block and has been used  
in various forms %, implicitly or explicitly, 
%has been used as an important building block 
in the design of many well-known algorithms, e.g., Quicksort~\cite{quicksort}, 
median~\cite{blummedian} and selection~\cite{blumselect,expectedselect,onfrselect}, 
and so on~\cite{parallelhash,parallelintegersorting,osortsmallkey,leightonselection}. 
%\elaine{cites}
Due to its close relationship to sorting, it has been investigated  
extensively often in conjunction with sorting~\cite{parallelhash,parallelintegersorting,osortsmallkey,leightonselection}.


Obviously, $n$ elements can be compacted 
can in $O(n)$ time on a Random-Access Machine (RAM) assuming
that each element fits in a memory word: one can make a linear scan
over the input array and whenever a distinguished element is encountered, write
it to an output array (and the same can be repeated for the non-distinguished elements).  
Somewhat surprisingly, however, the following fundamental and natural question 
has remained unanswered:
\begin{itemize}
\item[]
Does there exist a {\it circuit} family with $O(n \cdot w)$ 
number of AND, OR, and NOT gates  
that correctly compacts any input array containing $n$ elements each of 
$w$ bits\footnote{Note that at least $\Theta(n \cdot w)$ 
gates are necessary since 
even writing down the answer takes at least $n \cdot w$ bits; and 
moreover, in general we cannot reuse an input wire as an output wire --- otherwise
it would not be too hard to construct an input for which the output will be wrong.}?
\end{itemize}

%At first sight the question might seem simple; although  
Despite the superficial simplicity of the problem statement, 
one soon realizes that the answer it begs is likely highly non-trivial
from a technical perspective --- as we explain below, 
several natural classes of solutions are immediately ruled out.
A first observation is that 
the aforementioned simple RAM algorithm for compaction 
cannot be easily implemented as a linear-sized circuit since its memory accesses
are input-dependent. 
Secondly, observe that any comparison-based circuit cannot work --- due
to the well-known 0-1 principle~\cite{zeroone}, %\elaine{cite} 
any {\it comparison-based} circuit 
that correctly sorts an input array with 0/1 keys 
can also sort input arrays with arbitrarily long keys; and thus
the  $\Omega(n \log n)$ lower bound for comparison-based sorting would also apply 
to comparison-based compaction.
Last but not the least, another subtlety is that 
any ``natural'' compaction circuit 
cannot preserve {\it stability}, 
i.e., the output cannot preserve the relative ordering 
of distinguished elements as they appeared in the input (and the same 
holds for non-distinguished elements) --- this follows
from a lower bound proven by Lin, Shi, and Xie~\cite{osortsmallkey}
who showed that 
any {\it stable} compaction circuit that treats the elements as {\it indivisible}
(i.e., the circuit only moves the elements around through selector gates
and does not perform boolean computation on the encoding of the elements)
must be at least $\Omega(n \log n)$ in size.
Moreover, 
Afshani et al.~\cite{lbmult} showed the same lower bound but
removing the indivisibility assumption 
%and showed that {\it any} circuit 
%that {\it stably} compacts an input array must be at least $\Omega(n \log n)$ 
%in size
assuming that the well-known Li-Li network coding conjecture~\cite{lilinetcoding}
is true\footnote{This is not explicitly stated in their paper but is directly
implied by Theorem 2 of their paper.}.
%Notably, the circuit construction 
%in this paper in fact follows the indivisible assumption.

With these observations, we may refine the problem statement  
and ask instead whether 
compaction be solved with a linear sized circuit
by employing non-comparison-based techniques,
and moreover, by not insisting on preserving stability.

Perhaps due to the aforementioned natural barriers, it turns out that
our knowledge of this seemingly simple problem is relatively little.
%despite the  simplicity of the problem statement! 
To the best of our knowledge, 
to date the best-known {\it explicit} solution 
is none other but {\it sorting} itself! 
Using a sorting circuit (e.g., AKS~\cite{aks} or 
Zigzag sort~\cite{zigzag}), we can, of course, compact the input array, but consuming 
as many as $\Theta(n w \log n)$ gates.
Moreover, from what we know, most likely sorting is a 
strictly more difficult than compaction, and any 
endeavor to solve linear-sized compaction
by upgrading the problem to general sorting will unlikely succeed.
Specifically, a combination of 
recent works~\cite{sortinglbstoc19,lbmult,isthereoramlb} suggest  
that 
%solving  compaction through general sorting 
%is unlikely to yield a linear-sized circuit (even with 
%non-comparison-based techniques) --- combining the results of 
%Farhadi et al.~\cite{sortinglbstoc19} and Boyle and Naor~\cite{isthereoramlb},
%we know that sorting circuits 
sorting circuits of $o(w n \log n)$ size do not to exist~\cite{sortinglbstoc19,lbmult} 
if the famous Li-Li network coding conjecture 
is true~\cite{lilinetcoding} (and proving an unconditional lower bound 
has so far thwarted all our efforts).

%Despite the lack of explicit solutions besides sorting, we observe 
%that a non-trivial result can in fact be obtained by 
\paragraph{A warmup scheme.}
We observe 
that in fact, with some extra work, there is a way to tailor Pippenger's 
elegant self-routing superconcentrator construction~\cite{selfroutingsuperconcentrator} 
and implement it as an $O(n \log n + nw)$-sized circuit for compaction. 
To show this would involve some non-trivial techniques 
although arguably not the most interesting
part of our result.
We present this 
as a warmup scheme in Section~\ref{sec:firstattempt}
with non-trivial details deferred to Sections~\ref{sec:gadgets} and \ref{sec:tightfromloose}.
Notably, if $w \geq \log n$ the circuit would indeed be of $O(n w)$ size
(and indeed the circuit is non-comparison-based and does not preserve stability).
%Since Pippenger's work is described a different model of computation, to obtain
%the above circuit statement requires some extra work; thus we defer more discussions to 
%Section~\ref{sec:highlight}.
While this already seems like a big improvement 
in comparison with the na\"ive sorting-circuit baseline, 
the $O(n \log n + w n)$ bound is 
nonetheless somewhat unsatisfying. In particular, 
for the $w \in \left[\omega(1), o(\log n)\right]$ regime, 
the existence of a linear-sized compaction circuit still seems elusive, and to the
best of our knowledge such a result is not easily implied by 
the existing literature.


%how to implement his construction into a circuit model in 
%more detail in Section~\ref{sec:highlight}.


%To the best of our knowledge, no straightfoward modification 
%and straightforward modifications
%of Asharov's algorithm~\cite{optorama} do not seem to give such a result (although
%their work does provide a useful starting point for our work).
%\elaine{is this in fact already implied by pippenger's paper?}

\subsection{Main Result: Linear Compaction Circuit}

%\paragraph{Tight compaction circuit.}
In this paper, we show an asymptotic improvement regarding the size of 
compaction circuits, as stated in the following theorem:
%We show that indeed a linear-sized tight compaction
%circuit exists for almost all choices of $w$ leaving  
%only a tiny gap for future work. 

\begin{theorem}[Linear-sized tight compaction circuit]
For any arbitrarily small constant $\epsilon > 0$, 
there exists a circuit %of size $O(nw \poly (\log^*n - \log^* w))$ 
that can correctly compact 
any input array containing $n$ elements each of $w$ bits, and moreover
its size is upper bounded 
by 
\[
O(n w) \cdot \min\left( (\log^*n - \log^* w)^{2 + \epsilon}, \ \ 2^w/w \right)
\] 
As a direct corollary, if $w \geq \log^{(c)} n$
for any arbitrarily large constant $c \geq 1$ or if $w = O(1)$, 
then the circuit size is upper bounded by $O(n w)$.
\label{thm:introcompaction}
\end{theorem}
In the above, $\log^{(c)} m$
means taking iterated logarithm of $m$ for a total of $c$ times; and 
$\log^* m$ outputs the minimum $i$ such that $\log^{(i)} m \leq 1$.
Throughout the paper, $\log$ means $\log_2$ unless noted otherwise.

In essence, 
we show that indeed a linear-sized compaction circuit exists 
for almost all choices of $w$: when $w$ is at least  
$\log^{(c)} n$
for any constant $c$, 
or when $w$ is a constant.
%leaving only a tiny gap open for future work: specifically, 
%Our work leaves open the question whether a linear-sized
%tight compaction exists for the regime %$\omega(1) \leq w \leq \log^{(c)} n$
For the narrow regime 
when $w$ is super-constant but asymptotically smaller than
any $\log^{(c)} n$ for a constant $c$,  
%it remains unknown whether a linear-sized tight compaction circuit exists;
our solution is a $\min((\log^* n -\log^* w)^{2+\epsilon}, 2^w/w)$-factor away from optimal; and thus we leave open this tiny gap for a tiny regime for future work. 



\elaine{todo: double check the 2nd half of the min. also prove the second half 
in the technical section}

\ignore{
\paragraph{A note on stability.}
Our compaction circuit is {\it not stable}, i.e., 
the output does not preserve the 
relative ordering between distinguished (or non-distinguished) elements 
as they appeared in the input.
We note that this is inherent --- 
Lin, Shi, and Xie~\cite{osortsmallkey} proved that any ``natural'' circuit 
that treats each element as indivisible 
and {\it stably} compacts an input array 
must have size at least $\Omega(n \log n)$; 
Afshani et al.~\cite{lbmult} then removed the indivisibility assumption 
and showed that {\it any} circuit 
that {\it stably} compacts an input array must be at least $\Omega(n \log n)$ 
in size\footnote{This is not explicitly stated in their paper but is directly
implied by Theorem 2 of their paper.}.
Notably, the circuit construction 
in this paper in fact follows the indivisible assumption.
}

%\paragraph{A note on non-comparison-based techniques.}


%In this paper, we do not require the algorithm to be {\it stable}, 
%i.e., in the output, the relative ordering between the distinguished elements 
%can be arbitrary (and the same applies to non-distinguished elements).
%\elaine{need to explain this stability point}

\subsection{Additional Results: Selection and Sorting Elements with Small Keys}

\paragraph{Selection.}
Selection is the problem of selecting the $k$-th smallest element
or all $k$ smallest elements from an input array containing $n$ elements, each of $w$ bits.
Blum et al.~\cite{blummedian,blumselect}
described a linear-time algorithm for solving the selection 
problem in $O(n)$ time on a RAM assuming that the word size is at least $w$.
To select the $k$-th smallest element, 
the algorithm first divides the elements into $n/5$ groups each containing 5 elements, computes 
the median of each group, and then recursively computes the median of the medians
henceforth called a {\it pivot}.
At this moment, 
perform a {\it partitioning}:  
move all elements smaller than or equal to the pivot 
to the left and all other elements to the right and let ${\bf Y}$ be the resulting 
array.  Now, depending on the choice of $k$, recurse
on either the first $7n/10$ elements of 
${\bf Y}$ or the last $7n/10$ elements of ${\bf Y}$.

Somewhat surprisingly, it is not known how to construct a linear-sized
circuit for solving selection. Just like compaction, %from the literature 
partly the problem is that %there are some natural barriers towards accomplishing this 
natural classes of approaches break down: 
for example, it has been shown that any comparison-based 
{\it circuit} that selects $k$ smallest elements
%\elaine{TODO: check for which version of compaction this lb holds}
must incur at least $\Omega(n \log k)$ comparisons~\cite{leightonselection,sortminmem}\footnote{Note
that for sorting, the $\Omega(n \log n)$ comparison-based 
lower bound 
applies even to RAM algorithms; however, for selection, the
$\Omega(n \log k)$ comparison-based lower bound  
does not extend to RAM algorithms as demonstrated
by Blum et al.'s algorithm~\cite{blumselect,blummedian}.}.
Indeed, to the best of our knowledge, to date the 
best known (asymptotical) result for selection in the circuit model
is none other than sorting circuits~\cite{aks,zigzag}, i.e., incurring
$\Omega(w \cdot n \log n)$ number of gates. %, i.e., 
%asymptotically no better than using sorting circuit~\cite{aks,zigzag}. 
%\elaine{cite}
The selection problem has also been studied 
in other models of computation such as {\it probabilistic} circuit families~\cite{leightonselection}
and Valiant's parallel comparison-tree model~\cite{comparetree,pippengersortselect,beateigen}; 
%(see Section~\ref{sec:related} for details) \elaine{to write} --- 
however, %all these techniques
%do not directly lend themselves to computing the selection problem in circuit. 
these computing models are incomparable to circuits 
and do not directly imply $o(w \cdot n \log n)$ circuit-based results.

%\elaine{edit}
%We show how to construct a linear-sized 
Our techniques imply a linear-sized, non-comparison-based
selection circuit 
for almost all parameter regimes.
The key is to see that in Blum et al.~\cite{blumselect,blummedian}'s algorithm, 
the partitioning step can be accomplished with a compaction circuit.
Finally, if we can select the $k$-th smallest element, we can 
rely on compaction to 
find all $k$ smallest elements too.
Summarizing the above, %as a direct corollary, 
we get the following corollary:

\begin{corollary}[Linear-sized selection circuit]
For any arbitrarily small constant $\epsilon > 0$, 
there exists a circuit %of size $O(nw \poly (\log^*n - \log^* w))$ 
that can select the $k$-th smallest element or all $k$ smallest elements 
given any input array
containing $n$ elements each of $w$ bits;
%correctly compact 
%any input array containing $n$ elements each of $w$ bits, 
and moreover
its size is upper bounded 
by 
\[
O(n w) \cdot \min\left( (\log^*n - \log^* w)^{2 + \epsilon}, \ \ 2^w/w \right)
\] 
Specifically, if $w \geq \log^{(c)} n$
for any arbitrarily large constant $c \geq 1$ or if $w = O(1)$, 
then the circuit size is upper bounded by $O(n w)$.
\end{corollary}

\paragraph{Sorting elements with small keys.}
Using compaction and 
selection circuits as a building block, 
we in turn show the following:

\begin{corollary}[Sorting elements with small keys]
Let $\epsilon > 0$
be an arbitrarily small constant.
$n$ elements 
each $w$-bit in length and tagged with a $k$-bit key can be sorted
by a boolean circuit of 
size $O(n (w + k) \cdot k) \cdot (\log^* n - \log^*(w + k))^{2 + \epsilon}$.
\end{corollary}
For short keys $k < o(\log n)$ (ignoring $\poly \log^*$ terms),
this is asymptotically better than
any comparison-based approach which would suffer from an $\Omega(n (w+k) \log n)$
lower bound no matter how small $k$ is.
To prove this result, we build upon the techniques by 
Lin, Shi, and Xie~\cite{osortsmallkey} who constructed {\it randomized} algorithms
that sort elements with small keys (and thus their result is not in a circuit model). 
More specifically, their construction
leverages a carefully crafted two-parameter 
recursion. %but their approach is inherently randomized.  
We show that by leveraging (deterministic) compaction 
and selection as building blocks, we can replace the randomized components 
in Lin et al.~\cite{osortsmallkey}'s construction 
and still achieve roughly the same recurrence.
In comparison with Lin et al.~\cite{osortsmallkey},
not only do we make the algorithm deterministic, 
we also %improve their result asymptotically for 
achieve asymptotical improvements for 
$k < 2^{\log\log n/(\log^*n)^{2 + \epsilon}}$.
We thus answer another open question 
raised at the end of Lin et al.~\cite{osortsmallkey}.


%but with slightly better parameters. 






\section{Technical Highlight}
\label{sec:highlight}

%that this leads to an $O(n \log n + nw)$-sized circuit for compaction.
%will explain it in more 
%detail in Section~\ref{sec:highlight}. 
%the very recent work by Asharov et al.~\cite{optorama}.
%--- in this sense, 
%their work represents an exciting step forward in a direction that has long been stagnant.
%Specifically, they describe linear-time a deterministic 
%compaction algorithm in the Oblivious RAM model (i.e., the algorithm's memory
%accesses must be input-independent)\footnote{Note Asharov et al.~\cite{optorama} 
%the merged version of the works of Peserico~\cite{pesericocompact} and 
%Asharov et al.~\cite{optoramaold}.}.  
%Although their result is described for a RAM, 
%we observe that 
%with a little more work, %one can show that their tight compaction algorithm in fact  
%it is possible to implement their algorithm as an $O(n \log n + w n)$-sized circuit. 
%Notably, if $w \geq \log n$ the circuit would indeed be of $O(n w)$ size
%(and indeed the circuit is non-comparison-based and does not preserve stability).
%In this sense, the work of Asharov et al.~\cite{optorama}
%represents exciting and much-awaited progress in a direction that has been stagnant
%for several decades; 


\subsection{Warmup: From Pippenger's Super-Concentrator
 to $O(n \log n + nw)$-Sized Compaction Circuit}
\label{sec:firstattempt}
Pippenger~\cite{selfroutingsuperconcentrator} describes an $O(n)$-sized super-concentrator 
construction with $n$ sources and $n$ destinations, such that 
given any subset of $k$ sources and  
any subset of $k$ destinations, a set of vertice-disjoint paths 
exist between the sources and destinations. %(where each source can be matched
%with an arbitrary destination out of the $k$ subset). 
If one thinks of the $k$ sources as clients, 
and the $k$ destinations as servers, a super-concentrator
allows each client to receive service from a server 
over {\it congestion-free} paths. Note that all servers 
are assumed to 
provide the same type of service, and thus a client can be matched with any server.
Not only does Pippenger show the existence of vertice-disjoint 
paths between any $k$ sources and any $k$ destinations, importantly, 
he describes an explicit, efficient algorithm for 
finding a set of such paths when the $k$ sources and $k$ destinations 
have been specified --- henceforth we call this the {\it route-finding} algorithm.
%Such a super-concentrator is said to have an explicit 
%and efficient {\it route-finding} algorithm.


To use such a self-routing super-concentrator
to solve the compaction problem, 
one may think of the $k$ sources as the $k$ input elements
marked as distinguished, and the $k$ destinations as the first $k$  
positions of the output array, i.e., where the distinguished elements want to go.
Now, a trivial observation 
is that in Pippenger's construction,
the routing finding algorithm can be implemented as 
an $O(n)$-time RAM algorithm.  With some extra work, one can show
that in fact, the same route finding algorithm 
can be implemented as an $O(n \log n)$-sized
circuit: the detailed circuit construction 
involves a few non-trivial technicalities but
since this is not the most exciting part of our techniques, 
we defer the details to 
Sections~\ref{sec:lcprelim}, \ref{sec:lswprelim}, and \ref{sec:tightfromloose}.
%we will not spell out the detailed circuit construction  here 
%since our technical sections later in fact need to spell it out as a starting
%point of our bootstrapping and boosting technique. 
%Although the warmup scheme is not 
%the most interesting part of our construction, 
%we stress that a few non-trivial tricks are needed to show this

%but a detailed description is indeed contained in  
%our technical sections later. \elaine{refer}

Once the routes have been found, the $k$ distinguished elements 
can be routed to their respective destinations 
with an $O(n w)$-sized circuit.
This results in an $O(n\log n + nw)$-sized compaction circuit. 
%is not good enough to achieve our result stated earlier.
%which is the starting point of our final construction.

\paragraph{The usage of non-comparison techniques.}
At this moment we can reflect on how non-comparison-based techniques helped us
achieve this result which otherwise would have been impossible.
The warmup algorithm has a {\it metadata phase} 
(i.e., the route-finding phase) 
which involves
looking at only the distinguished/non-distinguished indicator of each element but not the elements themselves, 
and a {\it routing} phase that actually moves 
the elements around according to the plan computed by the metadata phase.
Importantly, 
the metadata phase makes the algorithm inherently non-comparison-based; and 
moreover,  
the cost of the metadata phase 
does not depend on $w$, i.e., the bit-width 
of the elements. 
The routing phase, on the other hand, moves $O(n)$ elements around  
since the super-concentrator 
is linear in size (and moving each element around incurs $O(w)$ number of gates 
when implemented in circuit).
This key insight will continue to help us throughout the remainder of the paper.


%\paragraph{Our approach.}
\subsection{A Slightly Deeper Dive into Pippenger's Construction}
\label{sec:pippenger}
% log^{. c}   C_0^{log c} = poly(c)
% c = log*n - log* w     

To explain our approach, it helps to dissect Pippenger's construction further.
For ease of understanding, we focus on achieving tight compaction, 
i.e., routing any $k$ positions in the input to the first $k$ positions in the output ---
but keep in mind that both Pippenger's and our 
construction can be generalized to %a self-routing super-concentrator capable of 
routing any $k$ positions in the input to any $k$ positions in the output.
Furthermore we explain their algorithm with 
a circuit computation model (although their original description is in a distributed
automata model). 

To achieve tight compaction,  
Pippenger first constructs a gadget capable of a relaxed form of compaction
henceforth called {\it loose compaction}.
In loose compaction, we have an input array of length $n$ where at most $n/128$
elements are {\it real} and the rest are {\it dummy}, 
and we would like to 
compress this array to half of the original size, while preserving
the multiset of real elements. 
Specifically, the loose compaction leverages a bipartite expander graph 
with $O(n)$ vertices 
where there are twice as many vertices on the left than on the right. \elaine{use this version?}
Each vertex has $O(1)$ edges. 
A route-finding
algorithm can be run to find a way to route the real elements on 
the left to the right without causing congestion, compressing
the array by a half in the process.
With a little more work, we show that it is possible to implement their route-finding
algorithm for loose compaction 
with an $O(n \log n)$-sized circuit (to be spelled out in Section~\ref{sec:lcprelim}). 
%\elaine{forward reference}
Once the routes have been found, the actual routing of the elements
from the left to the right 
can be accomplished with an $O(n w)$-sized circuit since the expander
graph has only $O(n)$ edges in total.

Given such a loose compaction gadget, Pippenger then upgrades it to tight compaction 
through non-trivial techniques, and the resulting
tight compaction preserves
the asymptotical cost of the loose compaction 
(the circuit variant of the upgrade will be 
spelled out in Section~\ref{sec:tightfromloose}).  \elaine{refer to later?}

\subsection{Our Approach in a Nutshell}
For simplicity, in the main body of the paper, we first present a construction
with a slightly looser $\poly\log^*$, i.e., not caring about the constant-degree of 
the $\poly(\cdot)$ function.
We shall tighten the constant-degree of the $\poly$ to $2+\epsilon$ in Appendix~\ref{sec:tighten}.

Let $\poly(\cdot)$
denote an appropriate polynomial function;
let $\alpha(n) \leq \log^* n$ any 
function that is upper-bounded by $\log^* n$ everywhere. 
%\gnote{it is not clear what appropriate function is} 
%and
%let $C > 2$ denote an appropriate constant. %that increases very slowly. 
Our construction (implicitly) builds  
an $\big(n %\cdot \log^{(\alpha)}) 
\cdot \poly(\alpha)\big)$-sized super-concentrator
with a routing-finding algorithm that can be implemented
as an $\big(n \cdot \log^{(\alpha)} n \cdot \poly(\alpha)\big)$-sized circuit.
Specifically, if we choose $\alpha(n) = \log^* n - \log^* w$, we have
an $\big(n \cdot \poly(\log^* n - \log^* w)\big)$-sized super-concentrator
whose routing-finding algorithm can be computed by  
an $\big(n w \cdot \poly(\log^* n - \log^* w)\big)$-size circuit.
In comparison with Pippenger's super-concentrator, we somewhat significantly 
reduce the size of the circuit implementing the routing-finding algorithm, 
at the price of a slightly super-linear super-concentrator.
%paying a slight price in the size of the super-concentrator.


\ignore{
The main cost to reduce is that of the route-finding algorithm.
A key insight is that the route-finding algorithm operates
only on metadata and not the input elements themselves.
}
The key insight is a 
new technique that involves repeated bootstrapping and boosting:
%non-trivial and novel recursion technique: 
we use loose compaction to bootstrap tight compaction 
with a constant blowup in circuit size;
%(this is done in the same
%fashion as Pippenger~\cite{selfroutingsuperconcentrator} but now in circuit);
then in turn, we use tight compaction 
to construct an asymptotically better loose compaction; and 
then in turn, we use the better loose compaction to bootstrap a better  
tight compaction, and so on.
See Figure~\ref{fig:demonstration} for a demonstration. 
More specifically,

\input{figure}
\begin{MyItemize}
\item {\it Tight compaction from loose compaction.}
Given a function $1 \leq f(n) \leq \log n$,
if loose compaction
can be accomplished with a $C_{\rm lc} \cdot (n f(n) + nw)$-sized circuit,
then we can accomplish tight compaction 
with a $C \cdot C_{\rm lc} \cdot (n f(n) + nw)$-sized circuit 
%(ignoring additive $O(n)$ factors) 
where $C$ and $C_{\rm lc}$ are suitable constants.
This uses 
the same techniques as in Pippenger's work but now applying them to the circuit model;


\item {\it Loose compaction from tight compaction.}
Let $f(n)$ be a function satisfying $1 \leq f(n) \leq \log n$,
and given a tight compaction circuit of $C_{\rm tc} \cdot (n f(n) + nw)$ size, 
we can construct a $C \cdot C_{\rm tc} \cdot (n f(f(n)) + nw)$-sized 
loose compaction circuit as follows where $C$ and $C_{\rm tc}$ are suitable constants:
\begin{enumerate}
\item 
Divide the input into chunks of $f(n)$ elements; for simplicity
we shall assume that $n$ is divisible by $f(n)$ here and the indivisible case
is handled later in our technical sections.
Mark chunks that have more than 
$f(n)/32$ real elements as {\it dense} and those with at most $f(n)/32$ 
real elements as {\it sparse}.

Use tight compaction to move all the dense chunks to the 
front and all the sparse chunks to the end.
Note that this step can be implemented as a $C_{\rm tc} (n + nw)$-sized circuit.

\item 
It is easy to show that there are at least $3n/4$ sparse chunks.
Now, for each of the trailing $3n/4$ sparse chunks,
use a tight compaction circuit
to compress away $31 f(n)/32$ dummy elements.
This step requires a $C_{\rm tc}\cdot (f(n) f(f(n)) + f(n) w)$-sized circuit 
per chunk and thus over all chunks, the total circuit size
is $\left(n/f(n)\right) 
\cdot  C_{\rm tc}\cdot (f(n) f(f(n)) + f(n) w) = C_{\rm tc}\cdot  (n f(f(n)) + nw)$.
\item 
The output is simply a concatenation of the following:
{\it i)} the first $n/4$ chunks; and {\it ii)} 
the remaining $f(n)/32$ elements for each of the remaining $3n/4$ chunks.  
It is not hard to show that the resulting array 
is less than half of the length of the original and no real element
is lost during this process.
\end{enumerate}
\end{MyItemize}

Now, as a starting point, we have a loose compaction 
circuit denoted $\LC_0$ whose size is $C_0 \cdot (n \log n + nw)$
for loosely compacting an input array of $n$ elements each of $w$ bits, where $C_0$ is
an appropriate constant --- as mentioned in Section~\ref{sec:pippenger},
we can construct such an $\LC_0$ using Pippenger's loose compactor construction but
implemennting his construction in a $O(n \log n + nw)$ involves some 
non-trivial technicalities which will be explained in Section~\ref{sec:gadgets}.
With $\LC_0$, we can construct a 
tight compaction circuit denoted $\TC_1$
of size at most $C \cdot C_0 \cdot (n \log n + nw)$.
Given $\TC_1$, we can in turn construct a loose compaction circuit 
denoted $\LC_1$ whose size is upper bounded by 
of size at most $C^2 \cdot C_0 \cdot (n \log \log n + nw)$.
Given  $\LC_1$, we can in turn construct a tight compaction
circuit denoted $\TC_2$ of size at most  
$C^3 \cdot C_0 \cdot (n \log  \log n + nw)$.
Given $\TC_2$, we can in turn construct a loose compaction
circuit denoted $\LC_3$ of size at most 
$C^4 \cdot C_0 \cdot (n \log^{(4)} n + nw)$.

Let $\alpha \leq \log^* n$, 
and let $2^{d-1} = \alpha$. 
After $d$
%after $d = \log \alpha$ 
iterations of the above recursion, we 
will obtain a tight compaction circuit $\TC_{d}$
whose size is upper bounded by 
%$\log^{(\alpha)} n$
$C^{2d-1} \cdot C_0 \cdot n \cdot (\log^{(2^{d-1})} n + w) 
= O(1) \cdot \poly(\alpha) \cdot n \cdot (\log^{(\alpha)} n + w)$.
Setting $\alpha = \log^*n - \log^* w$ would give us $\log^{(\alpha)}n = O(w)$ and thus we get 
a tight compaction
circuit of size 
$O(nw) \cdot \poly(\log^* n - \log^* w)$.


\ignore{
\begin{itemize}[leftmargin=5mm]
\item 
First, use an $O(n)$-sized expander 
graph to swap misplaced elements in the input, such that 
the remaining fraction of misplaced elements is bounded
by $1/128$.  
More specifically, 
if in the output, a position $i$ ought to contain a distinguished element
but in the input the position $i$ contains a non-distinguished element instead, then 
this element is colored ${\tt blue}$; 
contrarily, 
if in the output a position $i$ ought to contain a non-distinguished element
but in the input the position contains a distinguished element, then the
element is colored ${\tt red}$.
The total number of ${\tt blue}$ and ${\tt red}$ elements must be equal, and in this step
we use an expander graph to swap ${\tt blue}$ elements with ${\tt red}$ ones
such that the remaining density of  
misplaced elements is at most $1/128$. 

\item 
\end{itemize}
}



%in the language of compaction (although both their and our constructions 
%can be interpretted as a superconcentrator).
%To construct a linear-sized network 
%tight compaction, Pip

%\elaine{CONTINUE HERE}

\ignore{
Furthermore, he describes an algorithm for finding such vertice-joint paths
when the $k$ sources have been identified.
With some additional work, one can show that Pippenger's path-finding
algorithm can be implemented
as an $O(n\log n)$-sized circuit that is independent  
of the word-length $w$; and moreover 
once a set of paths have been identified, the routing of the elements
to the respective destinations can be accomplished with an $O(n w)$-sized circuit.
}



\subsection{Additional Related Work}
\label{sec:related}

%\elaine{tcc perfect oram paper, optorama, prob circuit family, results in valiant's model}

We now comment on additional related works. 
Specifically, several works 
have considered compaction and selection 
in other incomparable models of computation as explained below.
%that have not been mentioned before

Leighton et al.~\cite{leightonselection}
show how to construct comparison-based, {\it probabilistic} circuit families for selection, 
with $O(n \log \log n)$ comparators.
In their model, there is a family of circuits:
a random one is sampled without looking
at the input, and the sampled circuit must select the input array with high probability. 
One interesting observation 
is that although deterministic, comparator-based selection circuits
have a $\Omega(n \log n)$
lower bound~\cite{leightonselection,sortminmem}, probabilistic circuit families 
do not inherit the same lower bound.
Later works~\cite{osortsmallkey,odsmitchell} have improved Leighton's result and shown 
how to solve compaction 
either using probabilistic circuit families with $O(n \log \log n)$ comparators, 
or in $O(n \log \log n)$ time on a probabilistic Oblivious RAM.
Note that an Oblivious RAM is a RAM  
that requires the distribution of the algorithm's memory access patterns
to be input independent. 

A couple recent works have considered how to implement
(parts to all of) Pippenger's super-concentrator~\cite{selfroutingsuperconcentrator}
on a deterministic Oblivious RAM.
First, Chan et al.~\cite{perfectopram}
observe that Pippenger's loose compactor~\cite{selfroutingsuperconcentrator} (which
is arguably the most important building block in his super-concentrator)
has a route-finding algorithm that can be computed on an Oblivious RAM 
in $O(n \log n)$ time.
This was improved by   
Asharov et al.~in a very recent work~\cite{optorama},  %in a very recent work, 
where they show how to implement the route-finding algorithm for
Pippenger's entire super-concentrator (and not just the loose compactor part)
on an Oblivious RAM in $O(n)$ time.
Both Chan et al.~\cite{perfectopram} and Asharov et al.~\cite{optorama}
observe and make use of the fact that the route-finding algorithm  
operates only on metadata but not the input elements themselves; and in 
our work, we also leverage this insight 
to enable a new type of recursion that leads to our result.
We note that the Oblivious RAM model is incomparable to the circuit model
of computation, and thus %neither 
% Chan et al.~\cite{perfectopram} nor 
Asharov et al.~\cite{optorama}'s linear-time oblivious compaction scheme  
does not directly imply our result (and neither does our result imply theirs). 
In fact, %with some extra work (similar to the flavor in Section~\ref{sec:gadgets}), 
using the same techniques as in  Section~\ref{sec:gadgets},
one can show that 
Asharov et al.'s algorithm would still incur 
$O(n \log n + n w)$ cost if implemented as a circuit, i.e., no better than our 
warmup scheme in Section~\ref{sec:firstattempt}, obtained 
by directly implementing Pippenger's construction in circuit. 
This also suggests that Asharov et al.~\cite{optorama}
optimizations are tailored specifically for a RAM
model and does not lend directly towards a circuit construction.

Finally, sorting and selection have also been studied in the 
Parallel RAM (PRAM) model~\cite{parallelhash,parallelintegersorting,hanselection}
as well as in Valiant's comparison-based parallel 
computation model which charged only the comparisons but 
not the boolean computations that decided which elements to compare~\cite{comparetree,beateigen}. 









